Stabilizing Fast Dynamical Systems Using Time-of-Flight Cameras

Time-of-flight cameras are popular in robotics because they provide direct depth information and are compact, inexpensive, and less dependent on ambient visible light. However, their low spatial resolution and depth noise raise questions about their suitability for stabilizing fast, unstable dynamics. In this paper, we show that an inexpensive, low-resolution time-of-flight camera can provide angle feedback for reliable and precise balancing of an inverted pendulum on a cart, a canonical control benchmark. These results open the door to using compact, inexpensive, low-resolution time-of-flight cameras for precise feedback control of fast, unstable systems.

==> generated/paper_numbers.tex <==
\newcommand{\PaperCartMass}{\ensuremath{0.26}}
\newcommand{\PaperPendulumMass}{\ensuremath{0.015}}
\newcommand{\PaperPendulumLength}{\ensuremath{0.24}}
\newcommand{\PaperHingeDamping}{\ensuremath{2\times10^{-4}}}
\newcommand{\PaperGravity}{\ensuremath{9.81}}
\newcommand{\PaperTransmissionScale}{\ensuremath{-0.0399}}
\newcommand{\PaperGuidewayLengthMm}{\ensuremath{150}}
\newcommand{\PaperBeltWidthMm}{\ensuremath{6}}
\newcommand{\PaperPulleyTeeth}{\ensuremath{20}}
\newcommand{\PaperMotorEncoderBits}{\ensuremath{14}}
\newcommand{\PaperEncoderPulsesPerRev}{\ensuremath{600}}
\newcommand{\PaperCameraWavelengthNm}{\ensuremath{940}}
\newcommand{\PaperCameraWidth}{\ensuremath{240}}
\newcommand{\PaperCameraHeight}{\ensuremath{180}}
\newcommand{\PaperCameraRate}{\ensuremath{30}}
\newcommand{\PaperHostNodes}{\ensuremath{2}}
\newcommand{\PaperUartBaud}{\ensuremath{230400}}
\newcommand{\PaperControlRate}{\ensuremath{200}}
\newcommand{\PaperCartLimit}{\ensuremath{0.04}}
\newcommand{\PaperVelocityLimit}{\ensuremath{0.25}}
\newcommand{\PaperAngleInnovationLimit}{\ensuremath{0.35}}
\newcommand{\PaperLqrInputWeight}{\ensuremath{1}}
\newcommand{\PaperMinimumDepth}{\ensuremath{0}}
\newcommand{\PaperMaximumDepth}{\ensuremath{0.2}}
\newcommand{\PaperImageBits}{\ensuremath{8}}
\newcommand{\PaperMedianKernel}{\ensuremath{5}}
\newcommand{\PaperCropWidth}{\ensuremath{120}}
\newcommand{\PaperCropHeight}{\ensuremath{108}}
\newcommand{\PaperUpsampling}{\ensuremath{4}}
\newcommand{\PaperTipClearance}{\ensuremath{5}}
\newcommand{\PaperLoggingRate}{\ensuremath{50}}
\newcommand{\PaperBalanceDuration}{\ensuremath{60}}
\newcommand{\PaperComparisonDuration}{\ensuremath{600}}
\newcommand{\PaperTimingDuration}{\ensuremath{60}}
\newcommand{\PaperTimestampResolutionUs}{\ensuremath{1}}
\newcommand{\PaperTelemetryRate}{\ensuremath{200}}
\newcommand{\PaperVelocityLimitPadded}{\ensuremath{0.250}}
\newcommand{\PaperCanBitrateMbps}{\ensuremath{1}}
\newcommand{\PaperDriveControlRateKHz}{\ensuremath{8}}
\newcommand{\PaperComDistance}{\ensuremath{0.12}}
\newcommand{\PaperPivotInertia}{\ensuremath{2.88\times10^{-4}}}
\newcommand{\PaperGrowthTime}{\ensuremath{0.133}}
\newcommand{\PaperEncoderCounts}{\ensuremath{2400}}
\newcommand{\PaperEncoderStepDeg}{\ensuremath{0.15}}
\newcommand{\PaperAngleBinMrad}{\ensuremath{2.62}}
\newcommand{\PaperControlPeriodMs}{\ensuremath{5}}
\newcommand{\PaperCartBinMm}{\ensuremath{0.5}}
\newcommand{\PaperLqrWeightPosition}{\ensuremath{20}}
\newcommand{\PaperLqrWeightVelocity}{\ensuremath{1}}
\newcommand{\PaperLqrWeightAngle}{\ensuremath{1}}
\newcommand{\PaperLqrWeightAngularVelocity}{\ensuremath{1}}
\newcommand{\PaperBalanceTrials}{\ensuremath{10}}
\newcommand{\PaperBalanceSamples}{\ensuremath{3000}}
\newcommand{\PaperBalanceAngleRMSE}{\ensuremath{4.29}}
\newcommand{\PaperBalanceAngleMean}{\ensuremath{-0.721}}
\newcommand{\PaperBalanceCartRMSEmm}{\ensuremath{6.34}}
\newcommand{\PaperBalanceCartMeanMm}{\ensuremath{-3.28}}
\newcommand{\PaperBalanceRawDisagreement}{\ensuremath{3}}
\newcommand{\PaperBalanceFilteredDisagreement}{\ensuremath{2.8}}
\newcommand{\PaperComparisonEncoderAngleMean}{\ensuremath{-0.181}}
\newcommand{\PaperComparisonEncoderAngleRMSE}{\ensuremath{1.33}}
\newcommand{\PaperComparisonEncoderCartMean}{\ensuremath{-0.62}}
\newcommand{\PaperComparisonEncoderCartRMSE}{\ensuremath{1.09}}
\newcommand{\PaperComparisonTofAngleMean}{\ensuremath{-0.298}}
\newcommand{\PaperComparisonTofAngleRMSE}{\ensuremath{5.26}}
\newcommand{\PaperComparisonTofCartMean}{\ensuremath{-2.56}}
\newcommand{\PaperComparisonTofCartRMSE}{\ensuremath{5.34}}
\newcommand{\PaperComparisonSamples}{\ensuremath{30000}}
\newcommand{\PaperLightingLampDistanceCm}{\ensuremath{30}}
\newcommand{\PaperLightingTotalTrials}{\ensuremath{30}}
\newcommand{\PaperLightingGroups}{\ensuremath{3}}
\newcommand{\PaperLightingTrials}{\ensuremath{10}}
\newcommand{\PaperConfidencePercent}{\ensuremath{95}}
\newcommand{\PaperLightingMinRMSE}{\ensuremath{4.19}}
\newcommand{\PaperLightingMaxRMSE}{\ensuremath{4.41}}
\newcommand{\PaperLightingNormalIlluminance}{\ensuremath{500}}
\newcommand{\PaperLightingNormalFirst}{\ensuremath{1}}
\newcommand{\PaperLightingNormalLast}{\ensuremath{10}}
\newcommand{\PaperLightingNormalMean}{\ensuremath{4.27}}
\newcommand{\PaperLightingNormalLow}{\ensuremath{4.01}}
\newcommand{\PaperLightingNormalHigh}{\ensuremath{4.53}}
\newcommand{\PaperLightingLampIlluminance}{\ensuremath{2000}}
\newcommand{\PaperLightingLampFirst}{\ensuremath{11}}
\newcommand{\PaperLightingLampLast}{\ensuremath{20}}
\newcommand{\PaperLightingLampMean}{\ensuremath{4.41}}
\newcommand{\PaperLightingLampLow}{\ensuremath{4.19}}
\newcommand{\PaperLightingLampHigh}{\ensuremath{4.63}}
\newcommand{\PaperLightingDarkIlluminance}{\ensuremath{0}}
\newcommand{\PaperLightingDarkFirst}{\ensuremath{21}}
\newcommand{\PaperLightingDarkLast}{\ensuremath{30}}
\newcommand{\PaperLightingDarkMean}{\ensuremath{4.19}}
\newcommand{\PaperLightingDarkLow}{\ensuremath{4.01}}
\newcommand{\PaperLightingDarkHigh}{\ensuremath{4.36}}
\newcommand{\PaperJsdLogBase}{\ensuremath{2}}
\newcommand{\PaperJsdEdgeOffset}{\ensuremath{0}}
\newcommand{\PaperJsdWidthMultiplier}{\ensuremath{1}}
\newcommand{\PaperJsdMaxWidthMultiplier}{\ensuremath{4}}
\newcommand{\PaperJsdWidthMultipliers}{\ensuremath{1, 2, 4}}
\newcommand{\PaperJsdEdgeOffsets}{\ensuremath{-0.5, 0}}
\newcommand{\PaperJsdAngleBin}{\ensuremath{2.62}}
\newcommand{\PaperLightingAngleJsdMin}{\ensuremath{0.00115}}
\newcommand{\PaperComparisonAngleJsdSensitivityMin}{\ensuremath{0.0262}}
\newcommand{\PaperLightingAngleJsdMax}{\ensuremath{0.00278}}
\newcommand{\PaperComparisonAngleJsdSensitivityMax}{\ensuremath{0.315}}
\newcommand{\PaperComparisonAngleJsd}{\ensuremath{0.315}}
\newcommand{\PaperJsdCartBin}{\ensuremath{0.5}}
\newcommand{\PaperLightingCartJsdMin}{\ensuremath{0.0196}}
\newcommand{\PaperComparisonCartJsdSensitivityMin}{\ensuremath{0.371}}
\newcommand{\PaperLightingCartJsdMax}{\ensuremath{0.0394}}
\newcommand{\PaperComparisonCartJsdSensitivityMax}{\ensuremath{0.444}}
\newcommand{\PaperComparisonCartJsd}{\ensuremath{0.443}}
\newcommand{\PaperTofDelayMs}{\ensuremath{27.1}}
\newcommand{\PaperTofDelaySearchMinMs}{\ensuremath{-50}}
\newcommand{\PaperTofDelaySearchMaxMs}{\ensuremath{50}}
\newcommand{\PaperTofDelaySearchStepMs}{\ensuremath{1}}
\newcommand{\PaperTofDelayStdMs}{\ensuremath{3.2}}
\newcommand{\PaperTofDelayDuration}{\ensuremath{60}}
\newcommand{\PaperTofDelayInterval}{\ensuremath{6}}
\newcommand{\PaperTofDelayWindows}{\ensuremath{10}}
\newcommand{\PaperTofDelayEdgeGuard}{\ensuremath{0.2}}
\newcommand{\PaperCameraTimingFrames}{\ensuremath{1800}}
\newcommand{\PaperCameraAlgorithmMeanMs}{\ensuremath{5.28}}
\newcommand{\PaperCameraAlgorithmStdMs}{\ensuremath{1.74}}
\newcommand{\PaperCameraAlgorithmPHighMs}{\ensuremath{7.63}}
\newcommand{\PaperCameraSdkToWriteMeanMs}{\ensuremath{10.7}}
\newcommand{\PaperCameraSdkToWriteStdMs}{\ensuremath{2.79}}
\newcommand{\PaperTimingMedianMs}{\ensuremath{5}}
\newcommand{\PaperTimingZeroPercent}{\ensuremath{99.5}}
\newcommand{\PaperTimingMinIntervals}{\ensuremath{1799}}
\newcommand{\PaperLightingTableRows}{%
Normal room lighting & \PaperLightingNormalFirst{}--\PaperLightingNormalLast{} & \PaperLightingNormalMean{} & $[\PaperLightingNormalLow,\PaperLightingNormalHigh]$ \\
Strong lamp illumination & \PaperLightingLampFirst{}--\PaperLightingLampLast{} & \PaperLightingLampMean{} & $[\PaperLightingLampLow,\PaperLightingLampHigh]$ \\
Dark room & \PaperLightingDarkFirst{}--\PaperLightingDarkLast{} & \PaperLightingDarkMean{} & $[\PaperLightingDarkLow,\PaperLightingDarkHigh]$ \\
}

